DFormerv2: Geometry Self-Attention for RGBD Semantic Segmentation

Recent advances in scene understanding benefit a lot from depth maps because of the 3D geometry information, especially in complex conditions (e.g., low light and overexposed). Existing approaches encode depth maps along with RGB images and perform feature fusion between them to enable more robust predictions. Taking into account that depth can be regarded as a geometry supplement for RGB images, a straightforward question arises: Do we really need to explicitly encode depth information with neural networks as done for RGB images? Based on this insight, in this paper, we investigate a new way to learn RGBD feature representations and present DFormerv2, a strong RGBD encoder that explicitly uses depth maps as geometry priors rather than encoding depth information with neural networks. Our goal is to extract the geometry clues from the depth and spatial distances among all the image patch tokens, which will then be used as geometry priors to allocate attention weights in self-attention. Extensive experiments demonstrate that DFormerv2 exhibits exceptional performance in various RGBD semantic segmentation benchmarks. Code is available at: https://github.com/VCIP-RGBD/DFormer.

==> tabs/tab_main.tex <==
\begin{table*}[!t]
\centering
\caption{\textbf{Results on six multimodal semantic segmentation datasets}. The KITTI-360~\cite{liao2022kitti360} and our DeLiVER datasets have up to four modalities. The MFNet~\cite{ha2017mfnet} and NYU Depth V2~\cite{silberman2012nyuv2} datasets are dual-modal with respective RGB-Thermal and RGB-Depth modalities. The UrbanLF~\cite{sheng2022urbanlf} has up to 81 sub-aperture light-filed images. The quad-modal MCubeS dataset~\cite{liang2022mcubesnet} is for material segmentation.}
\vskip -1ex
\label{tab:res_all_six}
    \begin{minipage}[ht]{0.5\textwidth}
    \begin{subtable}{\linewidth}
    \caption{Results on KITTI-360 and \textsc{DeLiVER} datasets.}
    \label{tab:quad_modal}
    \setlength{\tabcolsep}{2pt}
    \resizebox{\columnwidth}{!}{    
    \renewcommand{\arraystretch}{1.22}
	\begin{tabular}{l|cc|c:c}
    \toprule
    \textbf{Method}& \textbf{Modal} & \textbf{Backbone} & \textbf{KITTI-360} & \textbf{DeLiVER} \\
    \midrule\hline
    HRFuser~\cite{broedermann2022hrfuser} & RGB & HRFormer-T  & 53.20 & 47.95 \\
    SegFormer~\cite{xie2021segformer} & RGB & MiT-B2 & 67.04 &  57.20 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser} & RGB-Depth & HRFormer-T &49.32 & 51.88\\
    TokenFusion~\cite{wang2022tokenfusion} & RGB-Depth & MiT-B2&  57.44 & 60.25\\
    CMX~\cite{liu2022cmx} & RGB-Depth & MiT-B2& 64.43 & 62.67\\
    \rowcolor{gray!15} CMNeXt & RGB-Depth & MiT-B2 & 65.09& 63.58 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser} & RGB-Event & HRFormer-T&44.85 & 42.22\\
    TokenFusion~\cite{wang2022tokenfusion} & RGB-Event & MiT-B2 & 55.97& 45.63 \\
    CMX~\cite{liu2022cmx} & RGB-Event & MiT-B2 & 64.03& 56.52\\
    \rowcolor{gray!15} CMNeXt & RGB-Event & MiT-B2 &  66.13& 57.48 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser} & RGB-LiDAR & HRFormer-T &48.74& 43.13\\
    TokenFusion~\cite{wang2022tokenfusion} & RGB-LiDAR & MiT-B2 & 54.55& 53.01\\
    CMX~\cite{liu2022cmx} & RGB-LiDAR & MiT-B2 & 64.31& 56.37\\
    \rowcolor{gray!15} CMNeXt & RGB-LiDAR & MiT-B2 &  65.26& 58.04 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser}& RGB-D-Event & HRFormer-T & 50.21& 51.83 \\
    \rowcolor{gray!15} CMNeXt & RGB-D-Event & MiT-B2 &  67.73& 64.44 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser}& RGB-D-LiDAR & HRFormer-T&52.61 & 52.72 \\
    \rowcolor{gray!15} CMNeXt & RGB-D-LiDAR & MiT-B2& 66.55 & 65.50 \\
    \hline
    HRFuser~\cite{broedermann2022hrfuser}& RGB-D-E-Li & HRFormer-T & 52.76& 52.97\\
    \rowcolor{gray!15} CMNeXt & RGB-D-E-Li & MiT-B2 & \textbf{67.84} & \textbf{66.30} \\
    \bottomrule
    \end{tabular}
    }
    \end{subtable}
    \end{minipage}%
    \begin{minipage}[ht]{\columnwidth}
    \begin{minipage}[ht]{0.55\columnwidth}
    \begin{subtable}{\linewidth}
    \centering
    \caption{Results on MFNet.}
    \label{tab:MFNet}
    \resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|c|c}
    \toprule
    \textbf{Method} & \textbf{Modal} & \textbf{mIoU}\\
    \midrule\hline
    SwinT~\cite{liu2021swin} & RGB & 49.0 \\
    SegFormer~\cite{xie2021segformer} & RGB & 52.0\\
    \hline
    ACNet~\cite{hu2019acnet} & RGB-T & 46.3 \\
    FuseSeg~\cite{sun2021fuseseg} & RGB-T & 54.5 \\
    ABMDRNet~\cite{zhang2021abmdrnet} & RGB-T & 54.8 \\
    LASNet~\cite{li2022lasnet} & RGB-T & 54.9 \\
    FEANet~\cite{deng2021feanet} & RGB-T & 55.3 \\
    MFTNet~\cite{zhou2022mftnet} & RGB-T & 57.3 \\
    GMNet~\cite{zhou2021gmnet} & RGB-T & 57.3 \\
    DooDLeNet~\cite{frigo2022doodlenet} & RGB-T & 57.3 \\
    CMX (MiT-B2)~\cite{liu2022cmx} & RGB-T & 58.2\\
    CMX (MiT-B4)~\cite{liu2022cmx} & RGB-T & 59.7\\
    % \hline
    \rowcolor{gray!15} CMNeXt (MiT-B4) & RGB-T & \textbf{59.9}\\
    \bottomrule
    \end{tabular}
    }
    }
    \end{subtable}
    \end{minipage}%
    \hspace{\fill}
    \begin{minipage}[ht]{0.44\columnwidth}
    \begin{subtable}{\linewidth}
    \centering
    \caption{Results on NYU Depth V2.}
    \label{tab:NYU}
    \resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|c}
    \toprule
    \textbf{Method} & \textbf{mIoU}  \\
    \midrule\hline
    ACNet~\cite{hu2019acnet} & 48.3 \\
    SGNet~\cite{chen2021sgnet}  & 51.1 \\
    ShapeConv~\cite{cao2021shapeconv} & 51.3  \\
    NANet~\cite{zhang2021nanet} & 52.3 \\
    SA-Gate~\cite{chen2020sagate} & 52.4  \\
    PGDENet~\cite{zhou2022pgdenet} & 53.7 \\
    \hline
    TokenFusion~\cite{wang2022tokenfusion} & 54.2 \\
    TransD-Fusion~\cite{wu2022transdfusion} & 55.5 \\
    MultiMAE~\cite{bachmann2022multimae} & 56.0 \\
    Omnivore~\cite{girdhar2022omnivore} & 56.8 \\
    CMX (MiT-B4)~\cite{liu2022cmx} & 56.3  \\
    CMX (MiT-B5)~\cite{liu2022cmx} & \textbf{56.9}  \\
    % \hline
    \rowcolor{gray!15} CMNeXt (MiT-B4) & \textbf{56.9} \\
    \bottomrule
    \end{tabular}
    }
    }
    \end{subtable}
    \end{minipage}
    \begin{minipage}[ht]{0.54\columnwidth}
    \begin{subtable}{\linewidth}
    \caption{Results on UrbanLF-Real and -Syn.}
    \label{tab:urbanlf}
    \resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{@{}l|c|cc@{}}
    \toprule
    \textbf{Method}& \textbf{Modal} & \textbf{Real} & \textbf{Syn} \\
    \midrule\hline
    PSPNet~\cite{zhao2017pspnet} & RGB  & 76.34 & 75.78\\
    OCR~\cite{yuan2020ocr} & RGB  & 78.60 & 79.36 \\
    SegFormer~\cite{xie2021segformer} (B4) & RGB & 82.20 & 78.53 \\
    \hline
    DAVSS~\cite{zhuang2020video} & Video &   75.91 & 74.27 \\
    TMANet~\cite{wang2021temporal} & Video & 77.14 & 76.41 \\
    \hline
    ESANet~\cite{seichter2021esanet}& RGB-D & \textit{n.a.} & 79.43\\
    SA-Gate~\cite{chen2020sagate} & RGB-D &  \textit{n.a.} & 79.53\\
    \hline
    PSPNet-LF~\cite{sheng2022urbanlf} & RGB-LF33 &  78.10 & 77.88\\
    OCR-LF~\cite{sheng2022urbanlf} & RGB-LF33 & 79.32& 80.43\\
    \rowcolor{gray!15} CMNeXt (MiT-B4) & RGB-LF8 & \textbf{83.22} & 80.74 \\
    \rowcolor{gray!15} CMNeXt (MiT-B4) & RGB-LF33 & 82.62 & 80.98 \\
    \rowcolor{gray!15} CMNeXt (MiT-B4) & RGB-LF80 & {83.11} & \textbf{81.02} \\
    \bottomrule
    \end{tabular}
    }}
    \end{subtable}
    \end{minipage}%
    \hspace{\fill}
    \begin{minipage}[ht]{0.45\columnwidth}
    \begin{subtable}{\linewidth}
    \caption{Results on MCubeS.}
    \label{tab:MCubeS}
    \resizebox{\columnwidth}{!}{
    \renewcommand{\arraystretch}{1.1}
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{@{}l|c|c@{}}
    \toprule
    \textbf{Method}& \textbf{Modal} & \textbf{mIoU} \\
    \midrule\hline
    DRConv~\cite{chen2021drconv} &RGB-A-D-N & 34.63 \\
    DDF~\cite{zhou2021ddf} &RGB-A-D-N & 36.16 \\
    TransFuser~\cite{prakash2021transfuser} &RGB-A-D-N & 37.66 \\
    MMTM~\cite{joze2020mmtm} &RGB-A-D-N & 39.71 \\
    FuseNet~\cite{hazirbas2016fusenet} &RGB-A-D-N & 40.58 \\\hline
    MCubeSNet~\cite{liang2022mcubesnet} &RGB & 33.70 \\
    \rowcolor{gray!15} CMNeXt (MiT-B2) &RGB & 48.16 \\ % 512x512
    MCubeSNet~\cite{liang2022mcubesnet} &RGB-A & 39.10 \\
    \rowcolor{gray!15} CMNeXt (MiT-B2) &RGB-A & 48.42 \\ % 512x512
    MCubeSNet~\cite{liang2022mcubesnet} &RGB-A-D & 42.00 \\
    \rowcolor{gray!15} CMNeXt (MiT-B2) &RGB-A-D & 49.48 \\ % 512x512
    MCubeSNet~\cite{liang2022mcubesnet} &RGB-A-D-N & 42.86 \\
    \rowcolor{gray!15} CMNeXt (MiT-B2) &RGB-A-D-N & \textbf{51.54} \\ % 512x512
    \bottomrule
    \end{tabular}  
    }}
    \end{subtable}
    \end{minipage}
    \end{minipage}
% 	\vskip-3ex
\vskip -1ex
\end{table*}
